DiVa: An Iterative Framework to Harvest More Diverse and Valid Labels from User Comments for Music

Towards sufficient music searching, it is vital to form a complete set of labels for each song. However, current solutions fail to resolve it as they cannot produce diverse enough mappings to make up for the information missed by the gold labels. Based on the observation that such missing information may already be presented in user comments, we propose to study the automated music labeling in an essential but under-explored setting, where the model is required to harvest more diverse and valid labels from the users' comments given limited gold labels. To this end, we design an iterative framework (DiVa) to harvest more $\underline{\text{Di}}$verse and $\underline{\text{Va}}$lid labels from user comments for music. The framework makes a classifier able to form complete sets of labels for songs via pseudo-labels inferred from pre-trained classifiers and a novel joint score function. The experiment on a densely annotated testing set reveals the superiority of the Diva over state-of-the-art solutions in producing more diverse labels missed by the gold labels. We hope our work can inspire future research on automated music labeling.

==> chapters/intro_old2.tex <==
\section{Introduction}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/demo.png}
    \caption{
    Illustration of (a) a song titled \textit{We Are The World}, (b) all possible labels of the song, and (c) the user comments of the song. The gold labels annotated by the expert only occupy part of all possible labels of the song. There lack of mappings to labels beyond the gold label vocabulary~(the issue of incomplete label coverage,  \plabel{touching}) and some labels in the gold label vocabulary~(the issue of incomplete supervision, e.g., \newsuper{hope}). Fortunately, such labels, including the gold ones~(e.g., \gold{classic}), may already be presented in the user comments of the song.
    }
    \label{fig:demo}
    \vspace*{-0.5cm}
\end{figure*}
Automated music labeling plays a vital role in music searching and recommendation. It enables us to represent different songs by different labels and helps users to easily find interested songs via these labels~\cite{hu2005mining,liang2018jtav}. A common solution is to hire experts to label the song based on the song metadata~(e.g., year) and their own knowledge. Despite being exact and widely used, such expert-generated labels are always too generalized to help users find songs they really desire. Take \textit{We Are The World} in \rfig{fig:demo} as an example, we fail to get it when searching with \gold{classic} on nearly all online music platforms ~(e.g., Spotify).
With the continually growing size of online music and the dynamically updating user searching preferences, industry-scale music searching \par
A helpful observation is that users themselves are ``experts'' in user searching. Specifically, the vocabulary the users used to comment on a song has a natural match to the vocabulary they used to search for the song~\cite{eck2007automatic}. Besides, the user comments, which are continuously updating because of the changing of user feelings on a song and the changing of Internet buzzwords, can indirectly reflect the dynamic changing of user searching preferences~\cite{mihret-atinaf-2019-sentiment}. This observation inspires us to harvest more labels from user comments. We believe such ``user-generated'' labels can largely enrich the expert-generated labels and support more sufficient music searching and recommendation. \par
In particular, instead of using user comments to predict labels, we prefer to harvest more labels from them. As the user comments are user-generated, and thus have a natural match to user searching behaviors. Besides, they are continuously accumulated, and thus have advantaged benefits to fit the dynamic changing of user searching preferences, compared to the metadata~(e.g., lyrics). As shown in \rfig{fig:demo}, given the gold labels and user comments, we want to harvest new supervision~(e.g., \newsuper{hope}) and new labels~(e.g., \plabel{unity}) from the user comments. Specifically, towards an accurate and complete representation of the song, we believe the newly generated labels should have two basic advantages. First, they should be sufficiently valid to serve as a label~(e.g., {\plabel{touching}} vs. \badlabel{that}) and to benefit music searching and recommendation~({e.g., \plabel{touching}} vs. \badlabel{melodious}). Second, they should be semantically different from each other including the gold ones to sufficiently cover the diverse music characteristics and user searching preferences of the song~(e.g., {\plabel{touching}} vs. \badlabel{moving}). \par
However, automated harvesting labels from user comments is not an easy job. Besides facing the issues of incomplete label coverage and incomplete supervision, it requires the labels to be diverse enough to cover different music information and user searching preferences and to be concise enough considering the storage and computation costs. This motivates us to propose the \name framework, which can produce ``user-generated'' labels for songs and contribute to covering more user searching preferences in a smaller vocabulary.
% \subsection{Intuition}
% Towards sufficient music searching and recommendation, it always pays to assign labels to a song. A common solution is to hire experts to label the song based on the song materials~(e.g., instruments) and their own knowledge. Despite being exact and widely used, such expert-generated labels are always too generalized to help the users find songs they really desire. Take \textit{We Are The World} as an example, we fail to get it when searching with \gold{classic} on nearly all music platforms ~(e.g., Spotify). A helpful observation is that users themselves are ``experts'' in user searching. Specifically, the vocabulary the users used to comment on a song has a natural match to the vocabulary they used to search for the song. Besides, the user comments, which are continuously updating because of the changing of user feelings on a song and the changing of Internet buzzwords, can indirectly reflect the dynamic changing of user searching preferences. This observation inspires us to harvest more labels from user comments. We believe such ``user-generated'' labels can largely enrich the expert-generated labels and support more sufficient music searching and recommendation. However, automated harvesting labels from user comments is not an easy job. Besides facing the issues of incomplete label coverage and incomplete supervision, it requires the labels to be diverse enough to cover different music information and user searching preferences and to be concise enough considering the storage and computation costs. This motivates us to propose the \name framework, which can produce ``user-generated'' labels for songs and contribute to covering more user searching preferences in a smaller vocabulary.
always requires a huge label vocabulary and an accurate and complete representation for each song based on the vocabulary~\cite{wei2022survey}. However, current multi-label classifiers~\cite{qin2019tuning,mersy2021efficient}, including the more advanced extremely multi-label learning methods~\cite{tagami2017annexml,guo2019breaking,wei2022survey}, fail to resolve this task because of the missing mappings from songs to labels in the annotated data.
Let's take a close look at the song~(\textit{We Are The World}) in \rfig{fig:demo}. Normally, the gold labels~(e.g., \gold{classic}) of a song are selected from a given label vocabulary by an expert based on the song materials and his own knowledge. However, such gold labels make up only part of all possible labels for a song due to two issues. First, there lack of mappings from songs to labels~(e.g., \plabel{unity}) that are suitable for the song but beyond the gold label vocabulary, namely, the issue of incomplete label coverage. This is because we cannot provide the annotator with a vocabulary covering all music characteristics and all user searching preferences, both of which keep changing over time. Second, even with a full label vocabulary, the mappings to some labels~(e.g., \newsuper{hope}) may also be missed by the expert, namely, the issue of incomplete supervision. This is because the expert can never be serious and careful enough to pinpoint all the right labels from thousands or more candidate labels in the vocabulary~\cite{xiong2022extreme}. Therefore, to achieve practical automated music labeling, a model needs to resolve the issues of incomplete label coverage and incomplete supervision comprehensively.\par
A few studies have made efforts to obtain new mappings using generative models~\cite{simig2022open} and self-training methods~\cite{zou2019confidence,xie2020self,xiong2022extreme}. However, we argue these studies cannot virtually resolve the above issues. As the newly mapped labels are either similar to the gold ones or copied from instances with similar features. So, such new labels can hardly provide more diverse information than the gold ones and cannot find all the missing mappings for the song. Hence, towards accurate and complete label representations for songs, we'd like to take a step forward and study automated music labeling in an essential but under-explored setting, where the model is required to find more \textbf{diverse} mappings from the song to labels beyond the gold label vocabulary and supervision missed by the experts. 
\par

To this end, we propose \name , which is an iterative framework to harvest more \underline{Di}verse and \underline{Va}lid labels for music. It is initialized with a binary classifier trained on user comments and gold labels. At this moment, the classifier is only capable to predict labels in the gold label vocabulary. We think this is because the mappings from the user comments to new supervision and new labels are missing during the training of the classifier. In other words, it will significantly promote the performance, if we retrain the classifier on the missing mappings. As a remedy, we leverage the complementary information from a joint score function that takes a unified look at the diversity and validness of a candidate label. In this way, we can obtain more diverse mappings to fine-tune the classifier. This process repeats several times until the classifier cannot predict any new mappings. We further collect a corpus from a Chinese online music platform. It consists of {16,372} songs, each of which consists of user comments and gold labels. Towards reliable evaluation, we also develop a testing set of label {1,000} songs, which have been densely annotated by experts based on the user comments. Experiment results show that, compared with state-of-the-art methods, the \name framework is more powerful in capturing more diverse labels and supervision than the state-of-the-art methods. We will release the dataset and codes to assist further studies once this paper is accepted. We hope our work can provide insights into automated music labeling and advance the research on incomplete label coverage and incomplete supervision in real-world applications.
In summary, we highlight our main contributions as follows.
\begin{itemize}
    \item {We call attention to the issues of incomplete label coverage and incomplete supervision in automated music labeling and take the first step to studying it in an essential but under-explored setting, where the model is required to produce more diverse mappings from songs to new labels and new supervisions.}
    \item We propose an iterative framework~(\name) to harvest more diverse and valid labels from user comments. It consists of a binary classifier and a joint score function. The classifier becomes more powerful gradually by fine-tuning on the pseudo-labels inferred from the previous classifier and the joint score function.
    \item The experiment reveals the superiority of \name in producing new labels beyond the gold label vocabulary and new supervision missed by experts. Further human evaluation also demonstrates that the \name can cover more user searching preferences because of the effectiveness gained by the joint score function.
    % with a smaller vocabulary.
\end{itemize}






% However, 
% However, automated harvesting labels from user comments is not an easy job. Current multi-label classifiers \cite{liang2018jtav,mersy2021efficient}, including the more advanced extremely multi-label learning methods~\cite{tagami2017annexml,guo2019breaking,wei2022survey}, fail to resolve this task because of the missing mappings from songs to labels in the annotated data.

% As far as we know, there lacks a 

% Hence, towards accurate and complete label representations for songs, we'd like to take a step forward and study automated music labeling in an essential but under-explored setting, where the model is required to find more \textbf{diverse} mappings from the song to labels beyond the gold label vocabulary and supervision missed by the experts. 
% \par


% We believe this problem can be greatly alleviated if we assign more diverse labels~(e.g., \plabel{unity}) to the song. As such, a
% Therefore, to achieve practical automated music labeling, a model needs to resolve the issues of incomplete label coverage and incomplete supervision comprehensively.


% The question is how to find more diverse labels given the gold labels and the gold label vocabulary. Current multi-label classifiers~\cite{liang2018jtav,mersy2021efficient}, including the more advanced extremely multi-label learning methods~\cite{tagami2017annexml,guo2019breaking,wei2022survey}, fail to resolve it as their prediction ab
% because of the missing mappings from songs to labels in the annotated data.





% With the continually growing size of online music and the dynamically updating user searching preferences, sufficient music searching, especially at the industrial scale, requires a large vocabulary involving all possible labels for all songs and an complete set of labels describing a specific song.\par



 
% Let's take a close look at the song~(\textit{We Are The World}) in \rfig{fig:demo}. Normally, the gold labels~(e.g., \gold{classic}) of a song are selected from a given label vocabulary by an expert based on the song materials and his own knowledge. However, such gold labels make up only part of all possible labels for a song due to two issues. First, there lack of mappings from songs to labels~(e.g., \plabel{unity}) that are suitable for the song but beyond the gold label vocabulary, namely, the issue of incomplete label coverage. This is because we cannot provide the annotator with a vocabulary covering all music characteristics and all user searching preferences, both of which keep changing over time. Second, even with a full label vocabulary, the mappings to some labels~(e.g., \newsuper{hope}) may also be missed by the expert, namely, the issue of incomplete supervision. This is because the expert can never be serious and careful enough to pinpoint all the right labels from thousands or more candidate labels in the vocabulary~\cite{xiong2022extreme}. Therefore, to achieve practical automated music labeling, a model needs to resolve the issues of incomplete label coverage and incomplete supervision comprehensively.\par
% A few studies have made efforts to obtain new mappings using generative models~\cite{simig2022open} and self-training methods~\cite{zou2019confidence,xie2020self,xiong2022extreme}. However, we argue these studies cannot virtually resolve the above issues. As the newly mapped labels are either similar to the gold ones or copied from instances with similar features. So, such new labels can hardly provide more diverse information than the gold ones and cannot find all the missing mappings for the song. Hence, towards accurate and complete label representations for songs, we'd like to take a step forward and study automated music labeling in an essential but under-explored setting, where the model is required to find more \textbf{diverse} mappings from the song to labels beyond the gold label vocabulary and supervision missed by the experts. 
% \par

==> tables/alg.tex <==
% \begin{algorithm*}
% \caption{Preprocessing procedure of \name}
%     \label{alg:pre}
% \KwData{user comments $\{X_i\}_{i=1}^N$, gold labels $\{\mathcal{Y}_i^G\}_{i=1}^N$,  pre-trained XLNet-base model~\cite{yang2019xlnet}}
% \KwResult{Representations of user comments and candidate labels}
% $\mathbb{Y}^G=\bigcup_{i=1}^{N}\mathcal{Y}_i^G$\;
% \For{$i\leftarrow 1$ \KwTo $N$}{
%     $\vec{X_i}$=XLNet$(X_i)$\;
%     $\mathcal{Y}_i= \mathcal{Y}_i^G$\;  
%     % \For{each $y^+$ in $\mathcal{Y}_i$}{
      
%     % }
% }
% candidate\_representations=$\{\}$
% \For{each $y_c$ in $\bigcup_{i=1}^{N}X_i\cup\mathbb{Y}^G$}{
%     $\vec{y_c}$=X2Static($y_c$, XLNet)\;
%     candidate\_representations $\leftarrow$ candidate\_representations$\cup \{y_c:\vec{y_c}\}$ 
% }
% Return $\{i: \vec{X_i}\}_{i=1}^N$, candidate\_representations
% \end{algorithm*}
\begin{algorithm*}
\small
\caption{The entire procedure of \name}
\label{alg:train}
\KwData{User Comments $\{X_i\}_{i=1}^N$, Gold Labels $\{\mathcal{Y}_i^G\}_{i=1}^N$,  Pre-trained XLNet-base Model~\cite{yang2019xlnet}, Hypeparameters}
\KwResult{Optimal Binary Classifier $\mathcal{F}$}
$\mathbb{Y}^G=\bigcup_{i=1}^{N}\mathcal{Y}_i^G$; \qquad \tcp{Preprocessing}
\For{$i\leftarrow 1$ \KwTo $N$}{
    $\vec{X_i}$=XLNet$(X_i)$; \qquad
    $\mathcal{Y}_i= \mathcal{Y}_i^G$\;  
}
\For{each $y_c$ in $\bigcup_{i=1}^{N}X_i\cup\mathbb{Y}^G$}{
    $\vec{y_c}$=X2Static($y_c$, XLNet)\;
}


Random initialize the parameters of binary classifier $\mathcal{F}$ defined by EQ.~(\ref{eq:ebc}); \qquad \tcp{Iteration}
\For{$m\leftarrow 1$ \KwTo Max\_Iteration}{ 

    Positive\_Data=\{\}; \qquad
    Negative\_Data=\{\}; \qquad \tcp{Data Preparation}
    \For{$i\leftarrow 1$ \KwTo $N$}{
    \textit{Candidates} = $X_i - \mathcal{Y}_i$\;
    \For{each $y^+$ in $\mathcal{Y}_i$}{
        Positive\_Data $\leftarrow$ Positive\_Data $\cup \{[{X_i},{y^+},1]\}$\;
         Random sample a $y^- \in$ \textit{Candidates}; \qquad
         Negative\_Data $\leftarrow$ Negative\_Data $\cup \{[{X_i},{y^-},0]\}$; \qquad
         \textit{Candidates} = \textit{Candidates}$-\{y^-\}$\;
    }
    }
    \textit{Train\_data} = Shuffle(Positive\_Data $\cup$ Negative\_Data); \qquad \tcp{Training}   
    
    \While{not converged}{
        $\mathcal{L}=0$\;
        \For{each $[x,y_c,y^*]$ in Train\_data}{
            Compute the confident score $\mathcal{F}({x,y_c})$; \qquad
            $\mathcal{L}=\mathcal{L}+BCE(y^*, \mathcal{F}({x,y_c})$)\;
        }
        Update the parameters of $\mathcal{F}$ based on $\mathcal{L}$\;
    }
    
    Pseudo\_Data=[]; \qquad \tcp{ $\mathcal{F}-$Inferring}
    \For{$i\leftarrow 1$ \KwTo $N$}{
    \textit{Candidates} = $X_i \cup \mathbb{Y}^G - \mathcal{Y}_i$; \qquad
    confidences=[]\;
    \For{each $y_c$ in \textit{Candidates}}{
         confidences=confidences.append($\mathcal{F}(X_i,y_c)$)\;
    }
    \For{each $\mathcal{F}(X_i,y_c)$ in Top\_K(confidences)}{
    \If{$y_c$ is not discarded on $\max(0,1-\sqrt{\alpha\times\frac{\sum u_{y_c}}{u_{y_c}}})$}
    {$\mathcal{Y}_i \leftarrow \mathcal{Y}_i \cup {y_c}$;  \qquad Pseudo\_Data=Pseudo\_Data.append($y_c$)\;}
    }
    
    }
    \eIf{Pseudo\_Data $\neq []$}{
      
       \textit{Candidates} = $X_i - \mathcal{Y}_i$; \qquad
        confidences=[]; \qquad \tcp{EQ.~(\ref{eq:joint})-Inferring}
    \For{each $y_c$ in \textit{Candidates}}{
          confidences=confidences.append($\mathcal{J}(y_c)$\;
    }
     \For{each $\mathcal{J}(y_c)$ in Top\_K(confidences)}{
        \If{$y_c$ is not discarded on $\max(0,1-\sqrt{\alpha\times\frac{\sum u_{y_c}}{u_{y_c}}})$}
    {$\mathcal{Y}_i \leftarrow \mathcal{Y}_i \cup {y_c}$;  \qquad Pseudo\_Data=Pseudo\_Data.append($y_c$)\;}
    }
      }{
      Return $\mathcal{F}$
      }
     
    
}
Return $\mathcal{F}$
\end{algorithm*}   
% }
    % % \While{not converged}{
        
    % % }

    % $\vec{X_i}$=XLNet($X_i$)\;
    % $\mathcal{Y}_i= \mathcal{Y}_i^G$\;
    % $\mathbb{X}=\bigcup_{i=1}^{N}X_i$\, $\mathbb{Y}^G=\bigcup_{i=1}^{N}\mathcal{Y}_i^G$\;
    % \For{each $y_c$ in $\mathbb{X}\cup\mathbb{Y}$}{
    %     $\vec{y_c}$=X2Static($y_c$)\;
    % $i=i+1$\;
    % }



    
    % $\Delta \mathbb{Y}= \bigcup_{i=1}^{N}\Delta Y_i$\;
    % \While{$\Delta \mathbb{Y}\ne \varnothing$}{
    
    % \qquad \tcp{Training} 
    % \While{not converged}{
    
    % }
    % \qquad \tcp{Inferring} 
    % \qquad \tcp{Scoring} 
    % % \qquad \tcp{Fine-tuning} 
    
    % }



==> tables/main_results_ol.tex <==
\begin{table*}[t]
    \centering
    \caption{Performance of all methods on \texttt{test}-1/\texttt{test}-2 w.r.t., precision~(P), recall~(R), F1, nDCG, PSP~\cite{jain2016extreme}, PSnDCG~\cite{jain2016extreme}, soft precision~(SP) defined by EQ.~(\ref{eq:softp}), soft recall~(SR) defined by EQ.~(\ref{eq:softr}), soft F1~(SF1), average number of new pseudo-labels per song~(NP), average number of new supervision per song~(NS), average number of new labels per song~(NL), and the vocabulary size of new labels harvested from use comments~($|\mathbb{Y}^+|$). We mark the values indicating the best performance in bold and the values indicating the second-best performance with underlines.}
    \scalebox{0.88}{
    \begin{tabular}{lccccccccccccc}
    \hline\hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{MLC } } && \multicolumn{2}{c}{\textbf{XML }} & &\multicolumn{3}{c}{\textbf{Soft matching }} &&\multirow{2}{*}{\textbf{Coverage}}\\ 
        \cline{2-5}\cline{7-8}\cline{10-12}
         & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{nDCG} && \textbf{PSP} & \textbf{PSnDCG} & &\textbf{SP} & \textbf{SR} & \textbf{SF1}&&\\ 
        \hline
        % \textbf{All positive} & 0.090/& 1.000/ & 0.163/ & 0.401/ & 0.125/ & 0.352/ & 0.172/ & ~ & ~  \\ 
        % \textbf{exact match} & 0.148/ & 1.000/ & 0.256/ & 0.523/ & 0.428/ & 1.600/ & 0.239/ & ~ & ~  \\ \hline
        \textbf{TF-IDF} & 0.02/0.22 & 0.09/0.27 & 0.02/0.20  &0.05/0.38 && 0.03/2.23 & 0.10/4.09 && 0.06/0.31 & 0.16/0.33 & 0.08/0.29 && \\  \hline
        % 31.78 & 5.43 & 30.40 & 17,924 \\  \hline
        \textbf{MLC} & 0.04/0.06 & 0.01/0.01 & 0.02/0.01 & 0.04/0.06 && 0.05/0.07 & 0.05/0.07 && 0.05/0.07 & 0.02/0.01 & 0.03/0.02 &&\\
        % 0.25&5.67&0&0 \\ 
        \textbf{LightXML~\cite{jiang2021lightxml}} & 0.41/0.87 & 0.49/0.23 & 0.41/0.36 & 0.54/0.88 && 0.45/1.27 & 0.42/1.27 && 0.44/0.88 &  0.52/0.28 & 0.49/0.41 && \\
        % 3.69&3.68 &0.01&1\\ 

        \textbf{EQ. (\ref{eq:ebc})} & 0.44/0.88 & 0.69/0.31 & 0.51/0.44 & 0.69/0.90 && 0.68/1.33 & 1.08/1.36 && 0.48/0.89 & 0.71/0.36 & 0.54/0.50 && \\
        % 4.45 & 4.53 & 0.01 & 10\\ 
        \textbf{nnPU~\cite{kiryo2017positive} w/ EQ. (\ref{eq:ebc})} & 0.07/0.24 & 0.98/0.74 & 0.13/0.36 & 0.65/0.72 && 0.11/0.59 & 0.93/1.42 && 0.13/0.31 & 0.98/0.77 & 0.22/0.44 && \\
        % 71.69 & 0.10 & 45.20 & 1,190\\
       \textbf{EQ.~(\ref{eq:joint})} & 0.18/0.55 & 0.90/0.63 & 0.37/0.58 & 0.47/0.62 && 0.41/1.28 & 0.68/1.41 && 0.33/0.60 & 0.68/0.67 & 0.42/0.62 && \\  
       % 22.80 & 17.61 & 5.19 & 1,770 \\ 
        \hline
        \textbf{GROOV~\cite{simig2022open}} & 0.51/0.88 & 0.41/0.17 & 0.43/0.27 & 0.30/0.24 && 0.33/0.28 & 0.20/0.30 && 
        - & - & - && \\  
        % 16.34 & 16.33 & 0.01 & 3 \\ 
        \textbf{ChatGPT~\cite{ouyang2022training}} & 0.13 & 0.14 & 0.11 & 0.13 && 0.10 & 0.11 && - & - & - && \\  
        % 9.92 & 2.39 & 7.53 & 5,303 \\ \hline
        \textbf{NST~\cite{xie2020self} w/ MLC} & 0.02/0.02 & 0.00/0.00 & 0.00/0.00 & 0.020/0.02 && 0.02/0.04 & 0.02/0.04 && 0.02/0.02& 0.00/0.00 & 0.00/0.00 &&\\  
        % & &0&0 \\ 
        \textbf{NST~\cite{xie2020self} w/ EQ. (\ref{eq:ebc})} & 0.31/0.79 & 0.78/0.46 & 0.42/0.56 & 0.59/0.81 && 0.44/1.28 & 0.85/1.27 && 0.35/0.81 & 0.78/0.50 & 0.47/0.60 && \\  
        % 9.78 & 9.78 & 0.01 & 3 \\
        \hline
        \textbf{\name -static} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&& \\ 
        \textbf{\name -light}  & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&& \\ 
        \textbf{\name} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&& \\  \hline\hline
        % \textbf{EQ. (\ref{eq:ebc})\dag} & 0.031/0.040 & 0.976/0.860 & 0.060/0.076 & 0.452/0.445 && 0.042/0.056 & 0.605/0.607 && 0.134/0.153 & 0.980/0.889 & 0.235/0.261 & \\
        %  \textbf{nnPU~\cite{kiryo2017positive} w/ EQ. (\ref{eq:ebc})\dag} & 0.081/0.018 & 0.520/0.208 & 0.138/0.033 & 0.379/0.110 && 0.353/0.023 & 2.027/0.138 && 0.179/0.108 & 0.599/0.339 & 0.274/0.161 & \\ 
        %  \textbf{EQ.~(\ref{eq:joint})}\dag & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
        %  \textbf{NST~\cite{xie2020self} w/ EQ. (\ref{eq:ebc})\dag} & 0.038/0.044 & 0.934/0.832 & 0.073/0.084 & 0.495/0.482 && 0.051/0.061 & 0.641/0.638 && 0.142/0.158 & 0.946/0.863 & 0.247/0.267 & \\ 
        %  \textbf{\name -static\dag} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
        % \textbf{\name -inter\dag} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
        % \textbf{\name -light\dag}  & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
        % \textbf{\name\dag} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\  \hline\hline
    \end{tabular}
    }
    \label{tab:main-1}
\end{table*}
% \begin{table*}[t]
%     \centering
%     \caption{Performance of all methods on \texttt{test}-2. We mark the values indicating the best performance in bold.}
%     \begin{tabular}{lcccccccccccccccc}
%     \hline\hline
%         \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{MLC } } && \multicolumn{2}{c}{\textbf{XML }} & &\multicolumn{3}{c}{\textbf{Soft matching }} &&\multicolumn{4}{c}{\textbf{Diversity-based }}\\ 
%         \cline{2-5}\cline{7-8}\cline{10-12}\cline{14-17}
%          & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{nDCG} && \textbf{PSP} & \textbf{PSnDCG} & &\textbf{SP} & \textbf{SR} & \textbf{SF1}&&\textbf{PL}&\textbf{NS}&\textbf{NP}&$|\mathbb{Y}^+|$\\ 
%         \hline
%         % \textbf{All positive} & 0.090/& 1.000/ & 0.163/ & 0.401/ & 0.125/ & 0.352/ & 0.172/ & ~ & ~  \\ 
%         % \textbf{exact match} & 0.148/ & 1.000/ & 0.256/ & 0.523/ & 0.428/ & 1.600/ & 0.239/ & ~ & ~  \\ \hline
%         \textbf{TextRank} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&&\\ 
%         \textbf{EmbeddingRank} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{TF-IDF} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{EQ.~(\ref{eq:tf})} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ \hline
%         \textbf{MLC} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{LightXML~\cite{jiang2021lightxml}} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{GROOV~\cite{simig2022open}} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{EQ. (\ref{eq:ebc})} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{nnPU~\cite{kiryo2017positive} w/ EQ. (\ref{eq:ebc})} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ \hline
%             \textbf{NST~\cite{xie2020self} w/ MLC} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{NST~\cite{xie2020self} w/ EQ. (\ref{eq:ebc})} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ \hline
%         \textbf{\name -static} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{\name -inter} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{\name -light}  & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\ 
%         \textbf{\name} & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~ & &&&&&&& \\  \hline\hline
%     \end{tabular}
%     \label{tab:main-2}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Performance of all methods on \texttt{test}-1/\texttt{test}-2 w.r.t., precision~(P), recall~(R), F1, nDCG, normalized PSP~\cite{jain2016extreme}, normalized PSnDCG~\cite{jain2016extreme}, soft precision~(SP), soft recall~(SR), soft F1~(SF1), and the coverage score. We mark the values indicating the best performance in bold and the values indicating the second-best performance with underlines.}
    \scalebox{0.8}{
    \begin{tabular}{lccccccccccccc}
    \hline\hline
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{MLC } } && \multicolumn{2}{c}{\textbf{XML }} & &\multicolumn{3}{c}{\textbf{Soft matching }} &&\multirow{2}{*}{\textbf{Coverage}}\\ 
        \cline{2-5}\cline{7-8}\cline{10-12}
         & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{nDCG} && \textbf{PSP} & \textbf{PSnDCG} & &\textbf{SP} & \textbf{SR} & \textbf{SF1}&&\\ 
        \hline
        \textbf{TF-IDF} & 0.015/0.082 & 0.090/0.346 & 0.021/0.119  &0.046/0.247 && 0.061/0.404 & 0.057/0.342 && 0.064/0.245 & 0.164/0.415 & 0.081/0.282 && 0.139 \\  \hline
        \textbf{MLC} & 0.044/0.063 & 0.013/0.007 & 0.018/0.012 & 0.044/0.062 && 0.152/0.039 & 0.137/0.038 && 0.050/0.071 & 0.019/0.012 & 0.025/0.020 && 0.283 \\
        \textbf{LightXML~\cite{jiang2021lightxml}} & 0.405/0.819 & 0.488/0.271 & 0.411/0.396 & 0.539/\underline{0.834} && 0.449/0.123 & 0.418/0.116 && 0.441/0.877 &  0.521/0.316 & 0.449/0.454 && 0.395 \\

        \textbf{EQ. (\ref{eq:ebc})} & \underline{0.443}/\underline{0.836} & 0.691/0.360 & \textbf{0.510}/0.492 & \textbf{0.686}/\textbf{0.858} && 0.653/0.146 & \textbf{0.594}/0.135 && \textbf{0.475}/\textbf{0.893} & 0.713/0.404 & \textbf{0.544}/0.546 && 0.420 \\
        \textbf{nnPU~\cite{kiryo2017positive} w/ EQ. (\ref{eq:ebc})} & 0.070/0.189 & \textbf{0.980}/\underline{0.737} & 0.128/0.298 & \underline{0.654}/0.690 && 0.931/0.352 & 0.513/0.203 && 0.126/0.318 & 0.982/0.766 & 0.220/0.446 && 0.178 \\
       % \textbf{EQ.~(\ref{eq:joint})} & 0.000/0.422 & 0.000/0.400 & 0.000/0.399 & 0.000/0.454 && 0.000/0.574 & 0.000/0.431 && 0.025/0.608 & 0.091/0.456 & 0.068/0.511 &&0.438 \\  
        \hline
        \textbf{GROOV~\cite{simig2022open}} & \textbf{0.512}/\textbf{0.844} & 0.412/0.200 & 0.426/0.310 & 0.295/0.244 && 0.327/0.056 & 0.203/0.042 && - & - & - && 0.206
         \\   
        \textbf{ChatGPT~\cite{ouyang2022training}} & 0.128/0.270 & 0.141/0.098 & 0.110/0.129 & 0.130/0.177 && 0.105/0.069 & 0.105/0.070 && - & - & - && 0.239\\  \hline
        \textbf{NST~\cite{xie2020self} w/ MLC} & 0.096/0.155 & 0.022/0.013 & 0.034/0.024 & 0.098/0.155 && 0.189/-
        % 0.224 
        & 0.185/-
        % 0.224
        && 0.105/0.184& 0.029/0.021 & 0.044/0.037 && 0.286\\  
        \textbf{NST~\cite{xie2020self} w/ EQ. (\ref{eq:ebc})} & 0.337/0.775 & 0.746/0.483 & 0.444/0.584 & 0.603/0.802 && 0.645/-
        % 0.171
        & 0.462/-
        % 0.143
        && 0.378/0.841 & 0.765/0.521 & 0.487/0.633 && 0.484 \\  
        \hline
        \textbf{\name -static} & 0.175/0.566 & \underline{0.897}/\textbf{0.811} & 0.281/\underline{0.657} & 0.462/0.703 && \textbf{0.835}/-
        % \textbf{0.676}
        & 0.404/0.451 && 0.222/0.707 & 0.906/0.831 & 0.344/0.757 &&0.517 \\ 
        \textbf{\name -light}  & 0.367/{0.800} & 0.655/0.402 & \underline{0.447}/0.522 & 0.582/0.821 && 0.524/-
        % 0.174 
        & 0.419/0.143 && 0.404/0.867 & 0.680/0.445 & 0.486/0.576 && 0.450\\ 
        \textbf{\name} & 0.235/0.714 & 0.729/0.636 & 0.337/\textbf{0.662} & 0.574/0.775 && 0.646/-
        % 0.592 
        & 0.444/0.398 && 0.278/0.803 & 0.751/0.670 & 0.388/0.721 && 0.564\\  \hline\hline
    \end{tabular}
    }
    \vspace*{-0.2cm}
    \label{tab:main-1}
\end{table*}
